Zero-Shot Event Detection by Multimodal Distributional Semantic Embedding of Videos

We propose a new zero-shot Event Detection method by Multi-modal Distributional Semantic embedding of videos. Our model embeds object and action concepts as well as other available modalities from videos into a distributional semantic space. To our knowledge, this is the first Zero-Shot event detection model that is built on top of distributional semantics and extends it in the following directions: (a) semantic embedding of multimodal information in videos (with focus on the visual modalities), (b) automatically determining relevance of concepts/attributes to a free text query, which could be useful for other applications, and (c) retrieving videos by free text event query (e.g., "changing a vehicle tire") based on their content. We embed videos into a distributional semantic space and then measure the similarity between videos and the event query in a free text form. We validated our method on the large TRECVID MED (Multimedia Event Detection) challenge. Using only the event title as a query, our method outperformed the state-of-the-art that uses big descriptions from 12.6% to 13.5% with MAP metric and 0.73 to 0.83 with ROC-AUC metric. It is also an order of magnitude faster.

==> ASR_OCR_embedding2.tex <==
We detected OCR in videos using  ~\cite{myers2005rectification}.\ignore{The objective of the approach is to detect common
real-world instances of in-scene text such as street
signs, billboards, license plates, etc} Their method 
firstly rectifies a given region text by identifying its properties, then compute a corrective transformation, and finally recognizes the text. For ASR, we used~\cite{van2013extracting} to detect the speech in videos, where spoken concepts are processed by an ASR engine and acoustic concepts.
